Prompting Is All You Need: Automated Android Bug Replay with Large Language Models

Bug reports are vital for software maintenance that allow users to inform developers of the problems encountered while using the software. As such, researchers have committed considerable resources toward automating bug replay to expedite the process of software maintenance. Nonetheless, the success of current automated approaches is largely dictated by the characteristics and quality of bug reports, as they are constrained by the limitations of manually-crafted patterns and pre-defined vocabulary lists. Inspired by the success of Large Language Models (LLMs) in natural language understanding, we propose AdbGPT, a new lightweight approach to automatically reproduce the bugs from bug reports through prompt engineering, without any training and hard-coding effort. AdbGPT leverages few-shot learning and chain-of-thought reasoning to elicit human knowledge and logical reasoning from LLMs to accomplish the bug replay in a manner similar to a developer. Our evaluations demonstrate the effectiveness and efficiency of our AdbGPT to reproduce 81.3% of bug reports in 253.6 seconds, outperforming the state-of-the-art baselines and ablation studies. We also conduct a small-scale user study to confirm the usefulness of AdbGPT in enhancing developers' bug replay capabilities.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
We demonstrate the performance and usefulness of our approach \tool in Section~\ref{sec:evaluation} and Section~\ref{sec:userstudy}.
In this section, we investigate the favoring capability of the LLMs in automated bug replay and its potential value in software testing.

\subsection{Semantic and Syntactic Understanding}
In language, there are many ways to express the same thing in different words and different syntaxes, including synonyms, alternative phrasing, colloquial language, or even user's choice of expression (as discussed in Section~\ref{sec:rq1}).
This presents a critical challenge to previous natural language processing methods and language models~\cite{zhao2019recdroid,zhao2022recdroid+,zhang2023automatically,fazzini2018automatically}.
Large language models (LLMs), trained on ultra-large-scale corpora, offer tremendous potential in semantic and syntactic understanding from bug reports, as shown in the results in Section~\ref{sec:rq1}.
This is mainly due to the well-designed prompts and eliciting methods (e.g., chain-of-thought).
We believe our prompting engineering in LLMs introduces new possibilities for the bug reproduction and could play a bigger role in other software engineering tasks.


\subsection{Multi-Languages Understanding}
Results in Section~\ref{sec:rq2} have initially demonstrated the performance of our approach in addressing bugs in different languages.
This is because the LLMs are trained on a diverse set of texts in a variety of languages, e.g., at least 95 natural languages for ChatGPT~\cite{web:language}.
We elicit the language ability of LLMs to support the task of understanding bug reports in different languages.
More importantly, with this powerful ability, LLMs can be applied to many other fundamental software tasks that require language understanding, e.g., international software testing~\cite{wang2009locating,wang2010locating,wang2009transtrl} to distribute to different geographic regions with different languages across the world.
% crowdsource the bug reports with  different languages?

\subsection{GUI Testing}
GUI testing tools, such as probability-based or model-based~\cite{mao2016sapienz,gu2019practical,dong2020time}, often suffer from low testing coverage for automated app testing because of the complex and dynamic nature of GUIs~\cite{liu2022fill}, including sets of interactions and possible testing logic.
For example, to login an app, the testing tools need to first input the username and password fields, and then tap on the login button.
Results in Section~\ref{sec:rq2} have demonstrated the ability of LLMs in capturing dependencies among GUIs for guiding missing steps in the bug reports.
This potential could help the testing tools explore apps in a manner that mimics human users, in terms of testing the apps logically.
To this end, we would like investigate the implications of our prompt engineering of GUI guidance for the app testing in future research.


==> motivation1.tex <==
\section{Motivating Examples}
\label{sec:motivation}
In this section, we provide examples to illustrate the challenges of bug reports as studied in many previous works~\cite{bettenburg2008makes,zhang2023automatically,zhao2019recdroid}.
The overall status of these examples can clearly frame the context and motivation of this work and their characteristics will be taken into consideration in our approach prompt design.
But note that this motivational study just aims to provide initial examples towards developers supporting bug reports, and a more comprehensive empirical study would be needed to deeply understand it.

\begin{figure*}
	\centering
	\includegraphics[width = 0.95\textwidth]{figures/motivation1.png}
	\caption{Motivating examples of bug reports.}
	\label{fig:motivation}
\end{figure*}

\begin{figure}
	\centering
	\includegraphics[width = 0.65\linewidth]{figures/motivation2.png}
	\caption{Motivating examples of component mismatch.}
	\label{fig:motivation1}
\end{figure}

\subsection{S2R Extraction}
\label{sec:moti_subsec1}
Although the S2R in bug report is seemingly easy to parse for a human, the extraction will run into several problems when trying to do so automatically.
This is majorly due to the nature of human writing, which is inconsistent, ambiguous, and vague.

\textbf{Inconsistent Formats.}
Separating the steps in a bug report is not a trivial task.
The users may use different formats to compose the bugs depending on their writing preferences.
The common formats are numeric indexing, list indexing, or using commas in a line.
However, regarding their understanding of the bugs, they may compose the steps under the same state as shown in Figure~\ref{fig:motivation}-D, that the automatic approaches may fail to interpret them as separate steps.
% 3. different writing format

\textbf{Diversified Words.}
The users may use different words or phrases to describe the same concept, making it difficult for automatic techniques to recognize the semantic patterns.
This can include synonyms, alternative phrasing, or even colloquial language.
For example, as shown in Figure~\ref{fig:motivation}-E and \ref{fig:motivation}-F, the users colloquially use ``go to'', ``click'', ``choose'', ``open'', ``create'', ``select'' to refer to the action of ``tap''.
Even for the same word, the user's voice may affect the recognition, e.g., ``click the button'' and ``the button is clicked'' in Figure~\ref{fig:motivation}-G.
While prior approaches~\cite{zhao2019recdroid,zhao2022recdroid+} have identified some common vocabulary of words, the inconsistency of human words still poses challenges of recognizing diversified word patterns in the bug reports.
% 4. semantic understanding (attempt to, go to, view)

\textbf{Dependent Context.}
Context-dependency can occur at a macro perspective.
For example, in Figure~\ref{fig:motivation}-H, the users demonstrate an action of ``deleteing'' a value, which is equivalent to ``leave the EditText empty'', thus, they should be interpreted as one step.
In Figure~\ref{fig:motivation}-I, the users may omit the details by repeating the previous steps, such as ``repeat the step'', ``create another one'', etc.
However, without syntactic awareness, the automatic approaches may not monitor the relationships among the words in a sentence, causing inaccurate S2R extraction.

Context-dependency can also occur at a more granular level.
The users may use conjunction words to order the reproduction steps, that differ from their syntactic order.
Previous work~\cite{zhang2023automatically} proposes an automatic approach based on constituency grammar to deal with common connective words (i.e., ``before'', ``after'', ``when'', etc.), while it is limited to less commonly-used words.
For instance, in Figure~\ref{fig:motivation}-J, the action to ``Favorites settings'' should happen first and then the action to ``Show favorites above search bar'' due to the semantic of the connective word ``under'' between the steps, which the previous work fails to recognize.
% 1. syntactic challenge (leave the edittext to blank)
% 2. order (when, after, under)


\subsection{Guided Replay}
\label{sec:moti_subsec2}
Even assuming there is no noise in the S2R extraction, these approaches would still face challenges during reproduction when they try to automatically match S2Rs on the GUIs.

\textbf{Missing Steps.}
Missing steps in the bug reports are a key factor in failure to bug reproduction, even manually.
This might due to the users are usually non-technical, and they may not know how to write a complete bug S2R.
Without a complete set of instructions, the automatic approaches fails to reproduce the steps to trigger the bugs.
This can result in repetitive back and forth bug reporting or developers manually spend additional time and effort trying to explore the app and reproduce the bug~\cite{feng2022gifdroid}.
% First, the users  assuming that certain steps are obvious
% 2. missing steps


\textbf{Component Mismatch.}
There may be two possible reasons why S2R cannot directly match components on the GUI.
First, the users may express the component imprecisely.
For instance, the ``movie'' button is described as ``play the film''~\cite{zhao2019recdroid}, making the automatic approaches difficult to identify the exact GUI component to which the S2R refers.
Second, for multi-lingual testing, the languages of S2Rs and GUIs may be different.
Figure~\ref{fig:motivation1} shows an example that the user report the bug in English while it is reproduced on a GUI in French, causing the reproduction to fail.
% 1. keyword mapping (film, movie and different language, term)

\subsection{Motivation}
These examples confirm the challenges of bug reports, and motivate us to design an approach for automated bug replay.
One commonly-used practice for automated bug replay is natural language processing~\cite{zhao2019automatically,zhao2019recdroid,zhao2022recdroid+,fazzini2018automatically}.
To apply it, one need to manually observe the bug reports, construct a large-scale vocabulary of words, and develop crafted patterns for different types of bugs, which is extremely cost-expensive and effort-consuming. 
Nevertheless, it is limited to the diversity of the patterns.
Deep learning introduces more opportunities for the natural language process, but it requires massive of accurate bug reports to learn the characteristic of S2Rs. 


Taken in this sense, it is worthwhile to propose an approach to address these challenges of bug reports and at the same time need to be lightweight.
Inspired by the success of prompt engineering in natural language processing, we propose to prompt the large language models to extract the S2Rs and guide the bug replay.
As the LLMs are not specially designed for bug understanding, analysis, and replay, we propose novel methods to help the LLMs learn and apply to automated bug replay, such as few-shot learning and chain-of-thought reasoning.
Note that our approach does not require any training data and hand-crafted patterns, it is all driven by prompt engineering.







% 1. optional: positioning icon


